Learning with Preserving for Continual Multitask Learning

Artificial intelligence systems in critical fields like autonomous driving and medical imaging analysis often continually learn new tasks using a shared stream of input data. For instance, after learning to detect traffic signs, a model may later need to learn to classify traffic lights or different types of vehicles using the same camera feed. This scenario introduces a challenging setting we term Continual Multitask Learning (CMTL), where a model sequentially learns new tasks on an underlying data distribution without forgetting previously learned abilities. Existing continual learning methods often fail in this setting because they learn fragmented, task-specific features that interfere with one another. To address this, we introduce Learning with Preserving (LwP), a novel framework that shifts the focus from preserving task outputs to maintaining the geometric structure of the shared representation space. The core of LwP is a Dynamically Weighted Distance Preservation (DWDP) loss that prevents representation drift by regularizing the pairwise distances between latent data representations. This mechanism of preserving the underlying geometric structure allows the model to retain implicit knowledge and support diverse tasks without requiring a replay buffer, making it suitable for privacy-conscious applications. Extensive evaluations on time-series and image benchmarks show that LwP not only mitigates catastrophic forgetting but also consistently outperforms state-of-the-art baselines in CMTL tasks. Notably, our method shows superior robustness to distribution shifts and is the only approach to surpass the strong single-task learning baseline, underscoring its effectiveness for real-world dynamic environments.

==> 4_eval.tex <==
\section{Evaluation}
\label{sec:eval}

\subsection{Experiment Setup}
To validate our approach, we conduct a series of experiments designed not only to benchmark the performance of LwP but also to demonstrate the effectiveness of its core mechanism in Continual Multitask Learning (CMTL) scenarios. We begin by establishing LwP’s superior performance against state-of-the-art continual learning (CL) baselines across multiple datasets and modalities (Sec. \ref{sec:eval:comprehensive}). We then demonstrate a key advantage for real-world deployment: LwP’s enhanced robustness to distribution shifts, a critical challenge in dynamic environments (Sec. \ref{sec:eval:robustness}). To explain these results, we investigate the underlying reason for LwP’s success, showing how it mitigates catastrophic forgetting by preserving the geometric structure of the representation space—a claim supported by quantitative metrics like Backward Transfer (BWT) and qualitative visualizations (Section \ref{sec:eval:mitigating}). Finally, we validate our specific design choices through comprehensive ablation studies on our loss function and demonstrate the scalability of our method with larger models and higher-resolution inputs (Sec. \ref{subsec:effect_param_image_size} and \ref{subsec:ablation_results}).

\input{table_main}

Further details on the experimental setup, model architectures, baseline implementations, and additional results—including \rex{get rid of these dashes} a thorough comparison with Multitask Learning (MTL) methods, analysis on the impact of training sample size, and progression of the accuracy over time—are provided in the Appendix \ref{appendix:additional_result}.

% We present a set of experiments designed to rigorously validate our approach using three benchmark datasets that span multiple modalities. \textbf{1)} We conduct a comprehensive performance evaluation of our method, LwP, comparing it to state-of-the-art CL techniques. This assessment focuses on the average accuracy across all tasks after training is completed. \textbf{2)} We analyze the extent of catastrophic forgetting in each model, employing the Backward Transfer (BWT) metric \cite{BackwardTransfer} to quantify the accuracy degradation over successive tasks. \textbf{3)} We benchmark the effect of parameter and input sizes to demonstrate that LwP is scalable to both. \textbf{4)} We explore the effects of dynamic weighting and various distance/similarity functions, $d$, as proposed in other studies, on the performance metrics of LwP.



% Additionally, in the Appendix \ref{appendix:additional_result}, we explain a more detailed setup, including attributes, and conduct further evaluations through additional experiments. A thorough comparison with MTL methods is presented in Appendix \ref{appendix:MTL_comparison}. Furthermore, we supply supplemental diagrams that illustrate the progression of the accuracy over time for both the PhysiQ and FairFace datasets, which can be found in Appendix \ref{appendix:accuracy_progression}. Appendix \ref{appendix:training_sample} elaborates on the influence of the number of training examples on the overall performance of each model. 




%In Appendix \ref{appendix:ablation_results}, we explore the effects of dynamic weighting and various distance/similarity functions, $d$, as proposed in other studies, on the performance metrics of LwP. 
% In Appendix \ref{appendix:acc_per_iter}, we benchmark the rate of performance improvement per train iteration not only against other baseline CL models but also against MTL methods. Additionally, in Appendix \ref{appendix:mtltocl}, we explore training the first five tasks of the CelebA dataset using an MTL scheme, followed by a CL setting for the remaining five tasks.

\paragraph{Dataset} We utilize four datasets from two distinct modalities for our task-incremental learning experiments: BDD100K (object detection in driving scenes), CelebA (facial attribute recognition), PhysiQ (IMU-based exercise quality assessment), and Fairface (facial attribute recognition). Each dataset is structured into a series of tasks. Further details on each dataset, including the attributes, data splits, and preprocessing steps, are provided in the Appendix \ref{appendix:setup_cont}.


\paragraph{Baselines} Our primary emphasis is on CL baselines since integrating many MTL methods into CMTL often requires substantial modifications to accommodate the incremental characteristics of CMTL. For CL, we compare against Online Bias Correction (OBC) \cite{chrysakis2023online}, Dual View Consistency (DVC) \cite{Gu_2022_CVPR},  Dark Experience Replay (DER) \cite{buzzega_dark_2020}, DER++ \cite{boschini2022class}, Function Distance Regularization (FDR) \cite{benjamin_measuring_2019}, Experience Replay (ER) \cite{robins1995catastrophic,ratcliff1990connectionist}, Gradient-based Sample Selection (GSS) \cite{aljundi2019gradient}, online Elastic Weight Consolidation (oEWC) \cite{kirkpatrick_overcoming_2017}, Synaptic Intelligence (SI) \cite{zenke2017continual}, and Learning without Forgetting (LwF) \cite{li_learning_2017}. In addition, we compare our approach with MTL methods, which are detailed in  Appendix \ref{appendix:MTL_comparison}. These include the basic MTL approach of training all tasks simultaneously with different predictors \cite{caruana1997multitask}, as well as more advanced techniques like PCGrad \cite{yu2020gradient}, Impartial MTL (IMTL) \cite{liu2021towards}, and NashMTL \cite{navon2022multi}. We also include a single task learning (STL) baseline, where each task is learned separately. For the choice of distance metric $d$, we test common options such as Euclidean distance and cosine similarity, as well as loss functions designed to preserve relational knowledge, such as those proposed in RKD \cite{park_relational_2019} and Co2L \cite{cha_co2l_2021}. 

\paragraph{Model Architectures} We use a ResNet structure for the datasets \meiyi{What datasets? PhysiQ is not included in the datasets?}. Each task is predicted after a linear projection layer applied to the flattened last shared layer $\bm{z} \in \mathbb{R}^{512}$. Similarly, for PhysiQ, we use a 3-layer 1DCNN model with $\bm{z} \in \mathbb{R}^{128}$ final shared layer connected to task-specific linear layers. \meiyi{why this one is different? due to task? or to show your model's capability on different tasks?} We evaluate additional architectures and image sizes in Section \ref{subsec:effect_param_image_size}.

% \input{table_main}

\begin{figure*}[!t]
    \centering
    % First Subfigure
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/celeba_backward_transfer_diagram.png}
        \caption{CelebA}
        \label{Fig:celeba}
    \end{subfigure}
    % Second Subfigure
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/physiq_backward_transfer_diagram.png}
        \caption{PhysiQ}
        \label{fig:physiq}
    \end{subfigure} 
    % Third Subfigure
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/fairface_backward_transfer_diagram.png}
        \caption{FairFace}
        \label{fig:fairface}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/bdd100k_backward_transfer_diagram.png}
        \caption{BDD100k}
        \label{fig:bdd100k}
    \end{subfigure}
    
    \caption{Backward Transfer Diagrams for the Benchmark Datasets \meiyi{The figures are TOO small. Not readable.}}
    \label{fig:forward_info_loss_diagrams}
\end{figure*}

\subsection{Comprehensive Performance in CMTL} \label{sec:eval:comprehensive}
In this experiment, we evaluate the performance of our LwP against several state-of-the-art CL methods. All methods, except for LwF and LwP, are provided with a buffer size of 512 for the CelebA and FairFace datasets, and 46 for the PhysiQ dataset, corresponding to approximately 2-3\% of the training set for each dataset. Each model is trained five times using different random seeds. The standard training protocol consists of 20 epochs, with a batch size of 256 for image-based datasets and 32 for PhysiQ, coupled with early stopping. For PhysiQ, we only compare the average accuracy across the final task iteration due to the training instability caused by a smaller dataset size. Table \ref{tab:model_accuracy_combined} reports the average test accuracy, along with the standard deviation over five runs for each method and dataset. Fig. \ref{fig:selected_celeba_confusion_matrices} visualizes the progression of task accuracy in task iterations (left to right). Additional results are provided in Appendix \ref{appendix:accuracy_progression}

% \begin{figure*}[!htbp]
% \centering
% % LWP
% \begin{subfigure}[b]{0.13\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/cm/celeba_LWP_confusion_matrix.png}
%     \caption{LwP \textbf{Ours}}
%     \label{fig:selected_lwp}
% \end{subfigure}
% % LWF
% \begin{subfigure}[b]{0.13\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/cm/celeba_LWF_confusion_matrix.png}
%     \caption{LWF}
%     \label{fig:selected_lwf}
% \end{subfigure}
% % ER
% \begin{subfigure}[b]{0.13\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/cm/celeba_ER_confusion_matrix.png}
%     \caption{ER}
%     \label{fig:selected_er}
% \end{subfigure}
% % DVC
% \begin{subfigure}[b]{0.13\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/cm/celeba_OBC_confusion_matrix.png}
%     \caption{OBC}
%     \label{fig:selected_obc}
% \end{subfigure}
% \begin{subfigure}[b]{0.13\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/cm/celeba_DER_confusion_matrix.png}
%     \caption{DER}
%     \label{fig:selected_der}
% \end{subfigure}
% % DERPP
% \begin{subfigure}[b]{0.13\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/cm/celeba_DERPP_confusion_matrix.png}
%     \caption{DERPP}
%     \label{fig:selected_derpp}
% \end{subfigure}
% \begin{subfigure}[b]{0.13\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/cm/celeba_EWC_confusion_matrix.png}
%     \caption{oEWC}
%     \label{fig:selected_oewc}
% \end{subfigure}

% \caption{Selected matrices showcasing the accuracy progression for various models for the dataset CelebA. Each column corresponds to an iteration of the task, arranged sequentially from left to right. We generate confusion matrices normalized across all tasks for all models to ensure consistency. More details in Appendix \ref{appendix:additional_result}.}

% \label{fig:selected_celeba_confusion_matrices}
% \end{figure*}





Table \ref{tab:model_accuracy_combined} highlights that LwP consistently achieves superior performance across all three benchmarks and is the only method to exceed the Single Task Learning (STL) baseline. This suggests that other continual learning methods likely experience significant task interference. Additional results with MTL are provided in Appendix \ref{appendix:additional_result}. Furthermore, our approach is modality-agnostic, as evidenced by LwP's ability to generalize across different domains. This is demonstrated by the results on the PhysiQ dataset from the IMU sensor domain, which underscores LwP's robustness against challenges unique to non-image-based tasks.
\textit{The results suggest that LwP demonstrates competitive performance compared to existing continual learning methods across a range of benchmarks in CMTL settings. LwP consistently achieves higher accuracy than other approaches, including surpassing the STL baseline, which indicates its potential to reduce task interference and catastrophic forgetting across different modalities.} \rex{Higher accuracy does not necessarily mean the approach is better, especially under continual learning setups, right?}

\subsection{Robustness to Non-Stationary Task Distributions} \label{sec:eval:robustness}

For real-world applications, such as autonomous driving, a model must be robust not only to test-time shifts but also to scenarios where the training data itself is non-stationary. We leveraged the BDD100k dataset's rich annotations to design a CMTL protocol that explicitly simulates this challenge. 

Instead of training on the whole, mixed dataset, we created sequential tasks defined by shifting environmental conditions. For instance, in the 'Weather Shift' \rex{Review more carefully, if using AI to polish the paper, quotes and dashes make it very easy to tell} scenario, the model was trained sequentially on distinct tasks, where the data for each task came from a specific weather condition (e.g., Task 0: 'clear', Task 1: 'rainy', etc.). This protocol directly evaluates the model's ability to handle non-stationary input distributions ($P_{X}^{(t)} \neq P_{X}^{(t+1)}$).

The final three columns of Table \ref{tab:model_accuracy_combined} show the average accuracy of all models trained under these non-stationary protocols. While most models experience a significant performance drop when faced with compounding distribution shifts between tasks, LwP maintains a more significant advantage over the baselines. For instance, in the 'Weather Shift' scenario, LwP achieves an accuracy of 77.227\%, a notable performance gain compared to the next best model, FDR. This demonstrates that LwP learns more generalizable and fundamentally robust representations. By preserving the core latent structure, our method is less susceptible to catastrophic forgetting induced by shifting data distributions, a critical advantage for deploying intelligent systems in dynamic, real-world environments.


\subsection{Mitigating Forgetting by Preserving Representation Structure}\label{sec:eval:mitigating}

\begin{figure}[!htbp]
    \centering
   %originally .75
    \includegraphics[width=0.45\textwidth]{Figures/toy_example_horizontal.png}
    \caption{Impact of $\mathcal{L}_{\text{DWDP}}$ on a constructed example. After training on a concentric circle task ($y_2$), the representation space without our loss (left) degrades. With $\mathcal{L}_{\text{DWDP}}$ (right), the structure required for a subsequent XOR task ($y_1$) is preserved. \meiyi{The figures are TOO small. Not readable.}}
    \label{fig:toy_example}
\end{figure}


The Backward Transfer \cite{BackwardTransfer} is a metric to evaluate the influence of learning the current task on the performance of previous tasks. A positive backward transfer value indicates that, on average, accuracies on the previous tasks have increased during the current task iteration and vice versa. It is defined as:

\begin{equation}
    BWT = \frac{1}{T-1} \sum_{i=1}^{T-1} R_{T,i} - R_{i, i},
\end{equation}


where $T$ is the index of the current task, $i$ is an index of previous tasks ranging from $1$ to $T-1$, $R_{T,i}$ is the accuracy on task $i$ after training up to task T, and $R_{i, i}$ is the accuracy on task $i$  after learning. As illustrated in Fig. \ref{fig:forward_info_loss_diagrams}, we observe that LwP outperforms all baselines in terms of BWT across all benchmarks. This result is consistent with the visualization, where LwP can maintain the accuracy of each task since its initial training.

LwP's strong performance in backward transfer is not accidental; it is a direct consequence of its core mechanism. Unlike other methods that allow the feature space to drift, LwP actively preserves the geometric structure of the representation. This prevents the ``fragmentation" that causes catastrophic forgetting. The following visualizations demonstrate this principle in action. Figure \ref{fig:toy_example} illustrates this on a constructed dataset, where preserving the original cluster structure is essential for success on a subsequent task. Without $L_{DWDP}$ (left), this structure is lost; with it (right), the knowledge is preserved.

\subsection{Effect of Model Parameters and Image Sizes on Performance} \label{subsec:effect_param_image_size}

\begin{table}[!ht]
\centering
\small
\caption{Accuracy Percentage Comparison Across Models on CelebA Dataset (10 Task)}
\label{tab:celeba_model_accuracy}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l l c c c@{}}
\toprule
\shortstack{\textbf{Method} \\ \textbf{Type}} & \textbf{Model} & \shortstack{\textbf{ResNet50 } \\ ($32\times32$)} & \shortstack{\textbf{ResNet101} \\ ($32 \times 32$)} & \shortstack{\textbf{ResNet50} \\ ($224 \times 224$)} \\
\midrule
\multirow{10}{*}{CL}
& LwF & 59.277 $\pm$ 11.920 & 58.279 $\pm$ 11.202 & 60.012 $\pm$ 14.448 \\ 
& oEWC & 66.975 $\pm$ 10.110 & 67.159 $\pm$ 10.506 & 68.511 $\pm$ 13.352 \\
& ER & 65.335 $\pm$ 9.298 & 65.646 $\pm$ 8.784 & 65.973 $\pm$ 14.729 \\
& SI & 66.698 $\pm$ 10.030 & 67.456 $\pm$ 9.880 & 67.747 $\pm$ 13.754 \\
& GSS & 65.926 $\pm$ 13.120 & 65.587 $\pm$ 13.142 & 69.817 $\pm$ 18.771 \\
& FDR & 61.753 $\pm$ 11.943 & 61.720 $\pm$ 12.017 & 65.225 $\pm$ 15.545 \\
& DER & 62.105 $\pm$ 12.114 & 63.797 $\pm$ 10.774 & 69.859 $\pm$ 12.690 \\
& DERPP & 62.814 $\pm$ 11.071 & 62.957 $\pm$ 11.577 & 68.102 $\pm$ 13.557 \\
& DVC & 67.084 $\pm$ 10.380 & 65.340 $\pm$ 11.427 & 70.921 $\pm$ 13.823 \\
& OBC & 64.220 $\pm$ 11.237 & 66.058 $\pm$ 10.370 & 69.319 $\pm$ 13.607 \\
\midrule
\multirow{1}{*}{CMTL}
& \textbf{LwP} & \textbf{67.388 $\pm$ 11.125} & \textbf{69.432 $\pm$ 10.416} & \textbf{85.064 $\pm$ 5.388} \\
\bottomrule
\end{tabular}}
\end{table}



% resnet50
% lwp: experiment_results/CL/celeba/lwp/orig/dynamic/logs_10tasks_resnet50.pyd, 4
% der: experiment_results/CL/celeba/der/logs_10tasks_resnet50.pyd, 3

% \todo{TODO: reason why resnet50 and 101 not outperforming resnet18 on input size 32x32: probably overfitting issue}
Table \ref{tab:celeba_model_accuracy} illustrates that the LwP method scales effectively with increased input resolution and model size. We find that preserving the Gaussian kernel, as shown in eq. \ref{eq:loss_pres}, results in improved performance on larger scales, especially with respect to input resolution. In the ResNet50 benchmark utilizing a 224x224 image size, LwP notably surpasses other baselines by achieving an 85\% accuracy, which is about 15\% percentage points greater than the runner-up. This suggests that, as the input allows the model to create more insightful representations, LwP becomes increasingly advantageous because it can maintain these representations. We also note that the bigger models with the same input size are not performing as well as the one with ResNet18. This is because the inputs lack sufficient information to capture generalized patterns, leading to overfitting.

\subsection{Ablation Study}
\label{subsec:ablation_results}
\input{table_ablation}

To evaluate the impact of the proposed loss function, we perform experiments by selectively disabling the dynamic weighting feature and comparing it with other loss functions that also aim to preserve structures. In our evaluation, we include Co2L \cite{cha_co2l_2021}, RKD \cite{park_relational_2019}, and two novel variations of baselines: cosine similarity and the RBF kernel as described in eq. \ref{eq:loss_pres}.
%To the best of our knowledge, this is the first exploration of cosine similarity preservation and RBF kernel application in this context.

The results in Table \ref{tab:diff_loss} validate our specific design choices for the DWDP loss. The strong performance of the squared Euclidean distance underscores the importance of preserving the global structure of the representation. Furthermore, the consistent advantage gained by adding Dynamic Weighting confirms our hypothesis that selectively deactivating the preservation loss for inter-class pairs is crucial to avoid conflicts with class-separation objectives when learning new tasks.

==> Figures/forward_information_loss.tex <==
\begin{tikzpicture}
    \begin{axis}[
        ybar,
        bar width=0.25cm,
        width=6cm,
        height=5cm,
        enlarge x limits=0.15,
        ymin=-0.3, ymax=0.3,
        ylabel={\footnotesize Average Diff in Accuracy from t-1 to t},
        xlabel={\footnotesize Model},
        symbolic x coords={LWP, GSS, DER, FDR, DERPP, LWF},
        xtick=data,
        nodes near coords,
        every node near coord/.append style={font=\scriptsize, rotate=90, anchor=west},
        axis on top,
        grid=both,
        grid style={dashed, gray!30},
        ticklabel style = {font=\footnotesize},
        yticklabel style = {font=\footnotesize},
        title={Forward Information Loss Diagram (physiq)},
        title style={font=\footnotesize, yshift=-1ex},
        xtick distance=1,
        xticklabel style={rotate=0, anchor=north},
    ]

    % LWP
    \addplot[
        fill=green!60,
        error bars/.cd,
        y dir=both, y explicit,
        error bar style={line width=0.8pt, black},
    ] coordinates {
        (LWP, -0.0476) +- (0, 0.02)
    };

    % GSS
    \addplot[
        fill=red!60,
        error bars/.cd,
        y dir=both, y explicit,
        error bar style={line width=0.8pt, black},
    ] coordinates {
        (GSS, -0.0965) +- (0, 0.03)
    };

    % DER
    \addplot[
        fill=blue!60,
        error bars/.cd,
        y dir=both, y explicit,
        error bar style={line width=0.8pt, black},
    ] coordinates {
        (DER, -0.1047) +- (0, 0.01)
    };

    % FDR
    \addplot[
        fill=orange!60,
        error bars/.cd,
        y dir=both, y explicit,
        error bar style={line width=0.8pt, black},
    ] coordinates {
        (FDR, -0.2134) +- (0, 0.04)
    };

    % DERPP
    \addplot[
        fill=purple!60,
        error bars/.cd,
        y dir=both, y explicit,
        error bar style={line width=0.8pt, black},
    ] coordinates {
        (DERPP, -0.1241) +- (0, 0.02)
    };

    % LWF
    \addplot[
        fill=cyan!60,
        error bars/.cd,
        y dir=both, y explicit,
        error bar style={line width=0.8pt, black},
    ] coordinates {
        (LWF, -0.2573) +- (0, 0.05)
    };

    \end{axis}
\end{tikzpicture}

